QVLA: Not All Channels Are Equal in Vision-Language-Action Model's Quantization

The advent of Vision-Language-Action (VLA) models represents a significant leap for embodied intelligence, yet their immense computational demands critically hinder deployment on resource-constrained robotic platforms. Intuitively, low-bit quantization is a prevalent and preferred technique for large-scale model compression. However, we find that a systematic analysis of VLA model's quantization is fundamentally lacking. We argue that naively applying uniform-bit quantization from Large Language Models (LLMs) to robotics is flawed, as these methods prioritize passive data fidelity while ignoring how minor action deviations compound into catastrophic task failures. To bridge this gap, we introduce QVLA, the first action-centric quantization framework specifically designed for embodied control. In a sharp departure from the rigid, uniform-bit quantization of LLM-based methods, QVLA introduces a highly granular, channel-wise bit allocation strategy. Its core mechanism is to directly measure the final action-space sensitivity when quantizing each individual channel to various bit-widths. This process yields a precise, per-channel importance metric that guides a global optimization, which elegantly unifies quantization and pruning (0-bit) into a single, cohesive framework. Extensive evaluations on different baselines demonstrate the superiority of our approach. In the LIBERO, the quantization version of OpenVLA-OFT with our method requires only 29.2% of the original model's VRAM while maintaining 98.9% of its original performance and achieving a 1.49x speedup. This translates to a 22.6% performance improvement over the LLM-derived method SmoothQuant. Our work establishes a new, principled foundation for compressing VLA models in robotics, paving the way for deploying powerful, large-scale models on real-world hardware. Code will be released.

==> table.tex <==
\section{Quantizing Diffusion LLM}


\begin{table*}[!t]
\caption{
Model performance on general tasks under weight-only quantization.
}
\vspace{-10pt}
\begin{center}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|c|c|cccccccc}
\toprule
\textbf{Model}    & \textbf{Setting}            & \textbf{Method} & \textbf{WinoGrande} & \textbf{PIQA} & \textbf{ARC-C} & \textbf{ARC-E} & \textbf{Hellaswag} & \textbf{MMLU 5-shot} & \textbf{Avg} & \textbf{Drop} \\ \midrule
\multirow{5}{*}{\textbf{LLaDA-8B}}                                                                          
& FP Model                    & -               & 69.9                & 74.6          & 46.4           & 71.1  & 70.7     & 65.7     & 65.5  & -    \\ \cmidrule{2-11} 
& \multirow{2}{*}{W4A16 g128} & GPTQ            & 69.7                & 73.9          & 47.9           & 72.5  & 70.4     & 64.7     & 65.3  & \cellcolor{green!10}$\downarrow$ 0.3\% \\
&                             & AWQ             & 67.3                & 70.3          & 44.5           & 73.4  & 68.4     & 65.6     & 63.2  & \cellcolor{orange!10}$\downarrow$ 3.5\% \\ \cmidrule{2-11} 
& \multirow{2}{*}{W3A16 g128} & GPTQ            & 67.2                & 73.3          & 45.7           & 71.1  & 68.8     & 63.5     & 63.7  & \cellcolor{orange!10}$\downarrow$ 2.7\% \\
&                             & AWQ             & 66.4                & 69.2          & 42.8           & 71.8  & 66.4     & 64.0     & 61.8  & \cellcolor{red!10}$\downarrow$ 5.6\% \\ \midrule
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}LLaDA-8B\\ -Instruct\end{tabular}}}} & FP Model                    & -               & 70.2                & 71.3          & 54.3           & 75.9  & 68.6               & 64.0                 & 65.7          & - \\ \cmidrule{2-11} 
\multicolumn{1}{c|}{}                                                                                       
& \multirow{2}{*}{W4A16 g128} & GPTQ            & 69.2                & 74.2          & 54.8           & 77.5  & 68.3     & 63.4     & 66.0  & \cellcolor{green!10}$\uparrow$ 0.3\%       \\
\multicolumn{1}{c|}{}                                                                                       
&                             & AWQ             & 68.8                & 71.0          & 53.3           & 76.1  & 68.1     & 63.4     & 64.9  & \cellcolor{green!10}$\downarrow$ 0.1\% \\ \cmidrule{2-11} 
\multicolumn{1}{c|}{}                                                                                       
& \multirow{2}{*}{W3A16 g128} & GPTQ            & 67.4                & 73.7          & 50.7           & 76.4  & 66.7     & 62.1     & 64.1  & \cellcolor{orange!10}$\downarrow$ 2.4\% \\
\multicolumn{1}{c|}{}                                                                                       
&                             & AWQ             & 66.3                & 69.8          & 50.5           & 74.7  & 66.4     & 62.3     & 63.1  & \cellcolor{orange!10}$\downarrow$ 4.0\% \\ \bottomrule
\end{tabular}
}
\end{center}
% \vspace{-1.8em}
\label{tab:weight-only-general}
\end{table*}
















\begin{table*}[!t]
\caption{
Model performance on general tasks under weight-activation quantization.
}
\vspace{-10pt}
\begin{center}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{c|c|c|ccccccc}
\toprule
\textbf{Model}                                                                         & \textbf{Setting}      & \textbf{Method} & \textbf{WinoGrande} & \textbf{PIQA} & \textbf{ARC-C} & \textbf{ARC-E} & \textbf{MMLU} & \textbf{Avg} & \textbf{Drop} \\ \midrule
\multirow{7}{*}{\textbf{LLaDA-8B}}                                                     
& FP Model              & -               & 69.9                & 74.6          & 46.4           & 71.1           & 65.7          & 65.5         & -             \\ \cmidrule{2-10}
                                                                                       
& \multirow{3}{*}{W8A8} & SmoothQuant     & 67.7                & 70.8          & 45.5           & 70.5           & 65.0          & 63.9         & \cellcolor{orange!10}$\downarrow$ 2.5\%         \\
&                       & QuaRot          & 68.6                & 71.1          & 45.2           & 70.8           & 66.1          & 64.4         & \cellcolor{orange!10}$\downarrow$ 1.8\%         \\
&                       & DuQuant         & 67.9                & 70.4          & 45.9           & 71.4           & 66.0          & 64.3         & \cellcolor{orange!10}$\downarrow$ 1.9\%         \\ \cmidrule{2-10} 
& \multirow{3}{*}{W4A4} & SmoothQuant     & 49.4                & 58.8          & 29.2           & 40.9           & 27.1          & 41.1         & \cellcolor{red!10}$\downarrow$ 37.3\%        \\
&                       & QuaRot          & 63.4                & 68.1          & 43.7           & 69.2           & 61.8          & 59.2         & \cellcolor{red!10}$\downarrow$ 6.6\% \\
&                       & DuQuant         & 64.9                & 69.3          & 42.8           & 70.0           & 64.0          & 62.2         & \cellcolor{red!10}$\downarrow$ 5.1\%         \\ \midrule
\multirow{7}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}LLaDA-8B\\ -Instruct\end{tabular}}} & FP Model              & -               & 70.2                & 71.3          & 54.3           & 75.9           & 64.0          & 67.1         & -             \\ \cmidrule{2-10} 
& \multirow{3}{*}{W8A8} & SmoothQuant     & 69.6                & 72.1          & 53.5           & 75.9           & 64.0          & 67.0         & \cellcolor{green!10}$\downarrow$ 0.2\%         \\
&                       & QuaRot          & 69.1                & 71.3          & 54.1           & 76.2           & 64.1          & 67.0         & \cellcolor{green!10}$\downarrow$ 0.3\%         \\
&                       & DuQuant         & 68.8                & 71.8          & 54.6           & 76.2           & 63.6          & 67.0         & \cellcolor{green!10}$\downarrow$ 0.2\%         \\ \cmidrule{2-10} 
& \multirow{3}{*}{W4A4} & SmoothQuant     & 52.3                & 65.1          & 34.0           & 54.0           & 32.8          & 47.7         & \cellcolor{red!10}$\downarrow$ 29.0\%        \\
&                       & QuaRot          & 65.2                & 69.8          & 51.3           & 75.1           & 61.1          & 64.5         & \cellcolor{orange!10}$\downarrow$ 3.9\%         \\
&                       & DuQuant         & 66.4                & 72.2          & 52.7           & 74.8           & 61.2          & 65.4         & \cellcolor{orange!10}$\downarrow$ 2.5\%         \\ \bottomrule
\end{tabular}
}
\end{center}
% \vspace{-1.8em}
\label{tab:wa-general}
\end{table*}







\subsection{Ideal Quantization Bit Precision (RQ1)}

\paragraph{4-bit is the Recommended Choice for Weight-Only Quantization.}

We observe that both GPTQ and AWQ perform well on general commonsense QA and math tasks under 4-bit quantization (Table~\ref{tab:weight-only-general} and Table~\ref{tab:weight-only-math-code}). In most cases, the performance degradation remains within the \textit{negligible} to \textit{moderate} range (i.e., <4\%).
For example, 4-bit GPTQ-quantized LLaDA-8B-instruct slightly improves the average accuracy on six QA tasks from 65.7\% to 66.0\%, and shows only a minor drop of 0.6\% on the MATH and GSM8K benchmarks.
In contrast, reducing the quantization bit-width to 3-bit leads to a \textit{significant} performance drop, particularly on math and code generation tasks, as shown in Table~\ref{tab:weight-only-math-code}.
Therefore, we recommend 4-bit quantization as the standard configuration for weight-only quantization of diffusion-based LLMs. The development of more robust 3-bit quantization methods remains an open research direction.



\paragraph{Weight-Activation Quantization: 8-bit is Tolerable, While 4-bit Remains Challenging.}
As shown in Table~\ref{tab:wa-general} and Table~\ref{tab:wa-math-code}, quantizing LLaDA models to W8A8 results in only minor performance degradation, largely independent of the specific quantization method. This suggests that even simple techniques such as SmoothQuant are effective in mitigating activation outliers in LLaDA models, leading to nearly lossless quantized variants.
However, reducing precision to W4A4 introduces a sharp performance drop across most benchmarks. 
In the majority of cases, performance degradation exceeds the \textit{significant} threshold (>4\%). For instance, SmoothQuant experiences a drop of over 20\% across all evaluated tasks, indicating that the simple rebalancing between weights and activations is insufficient under low-precision settings for dLLMs.
The degradation is especially pronounced in base models, with accuracy drops exceeding 10\% on code generation tasks and math reasoning-heavy benchmarks.
These results highlight the difficulty of achieving effective 4-bit weight-activation quantization in dLLMs, and point to the need for more advanced techniques. Improving performance under this challenging setting remains an open research problem for the community.






\begin{table*}[!t]
\caption{
Model performance on mathematics and code tasks under weight-only quantization.
}
\vspace{-10pt}
\begin{center}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|l|c|cccc|cccc}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}}                                   & \multirow{2}{*}{\textbf{Setting}} & \multirow{2}{*}{\textbf{Method}} & \textbf{GSM8K (4-shot)} & \textbf{Math (0-shot)} & \multirow{2}{*}{\textbf{Avg}} & \multirow{2}{*}{\textbf{Drop}} & \textbf{HumanEval (0-shot)} & \textbf{MBPP (3-shot )} & \multirow{2}{*}{\textbf{Avg}} & \multirow{2}{*}{\textbf{Drop}} \\
\multicolumn{1}{l|}{}                                                                  &                                   &                                  & Gen Len 256             & Gen Len 256            &                   &            & Gen Len 512                 & Gen Len 512             &               &                \\ \midrule
\multirow{5}{*}{\textbf{LLaDA-8B}}                                                     
& FP Model                          & -             & 69.7        & 21.3       & 45.5     & -                                         & 32.9                        & 39.4                    & 36.2      & -                    \\ \cmidrule{2-11} 
& \multirow{2}{*}{W4A16 g128}       & GPTQ          & 68.5        & 21.3       & 44.9     & \cellcolor{orange!10}$\downarrow$ 1.4\%   & 28.7                        & 39.4                    & 34.0      & \cellcolor{red!10}$\downarrow$ 5.9\%    \\
&                                   & AWQ           & 67.4        & 20.6       & 44.0     & \cellcolor{orange!10}$\downarrow$ 3.2\%   & 29.9                        & 37.2                    & 33.5      & \cellcolor{red!10}$\downarrow$ 7.3\%    \\ \cmidrule{2-11}
& \multirow{2}{*}{W3A16 g128}       & GPTQ          & 63.3        & 13.4       & 38.4     & \cellcolor{red!10}$\downarrow$ 15.7\%   & 26.2                        & 35.4                    & 30.8      & \cellcolor{red!10}$\downarrow$ 14.8\%    \\
&                                   & AWQ           & 64.3        & 17.0       & 40.6     & \cellcolor{red!10}$\downarrow$ 10.7\%   & 28.1                        & 34.2                    & 31.1      & \cellcolor{red!10}$\downarrow$ 13.9\%     \\ \midrule
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}LLaDA-8B\\ -Instruct\end{tabular}}} & FP Model                          & -                                & 78.5                    & 33.5                   & 56.0        & -                   & 37.8                        & 37.4                    & 37.6                          \\ \cmidrule{2-11} 
& \multirow{2}{*}{W4A16 g128}       & GPTQ          & 78.8        & 32.4       & 55.6     & \cellcolor{green!10}$\downarrow$ 0.6\%   & 36.6                        & 33.8                    & 35.2      & \cellcolor{red!10}$\downarrow$ 6.4\%    \\
&                                   & AWQ           & 78.9        & 33.6       & 56.2     & \cellcolor{green!10}$\uparrow$ 0.5\%   & 37.1                        & 35.6                    & 36.4      & \cellcolor{orange!10}$\downarrow$ 3.2\%    \\ \cmidrule{2-11}
& \multirow{2}{*}{W3A16 g128}       & GPTQ          & 76.4        & 30.0       & 53.2     & \cellcolor{red!10}$\downarrow$ 5.0\%   & 34.2                        & 30.0                    & 32.1            & \cellcolor{red!10}$\downarrow$ 14.7\%    \\
&                                   & AWQ           & 76.3        & 30.1       & 53.2     & \cellcolor{red!10}$\downarrow$ 5.0\%   & 34.1                        & 31.8                    & 33.0            & \cellcolor{red!10}$\downarrow$ 12.4\%    \\ \bottomrule
\end{tabular}
}
\end{center}
% \vspace{-1.8em}
\label{tab:weight-only-math-code}
\end{table*}





\begin{table*}[!t]
\caption{
Model performance on mathematics and code tasks under weight-activation quantization.
}
\vspace{-10pt}
\begin{center}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{l|cc|cccc|cccc}
\toprule
\multirow{2}{*}{\textbf{Model}}                                                        
& \multirow{2}{*}{\textbf{Setting}} & \multirow{2}{*}{\textbf{Method}} & \textbf{GSM8K (4-shot)} & \textbf{Math (0-shot)} & \multirow{2}{*}{\textbf{Avg}} & \multirow{2}{*}{\textbf{Drop}} & \textbf{HumanEval (0-shot)} & \textbf{MBPP (3-shot )} & \multirow{2}{*}{\textbf{Avg}} & \multirow{2}{*}{\textbf{Drop}} \\
&                                   &                                  & Gen Len 256             & Gen Len 256            &                               &                                & Gen Len 512                 & Gen Len 512             &                               &                       \\ 
\midrule
\multirow{7}{*}{\textbf{LLaDA-8B}}                                                     
& FP Model                          & -                                & 69.7                    & 21.3                   & 45.5          & -                              & 32.9                        & 39.4                    & 36.2                          & -                     \\ \cmidrule{2-11} 
& \multirow{3}{*}{W8A8}             & SmoothQuant                      & 69.4                    & 20.2                   & 44.8          & \cellcolor{orange!10}$\downarrow$ 1.6\%                          & 27.4                        & 40.2                    & 33.8                       &  \cellcolor{red!10}$\downarrow$ 6.5\%                 \\
&                                   & QuaRot                           & 69.9                    & 20.7                   & 69.9          & \cellcolor{green!10}$\downarrow$ 0.4\%                      & 31.7                        & 40.6                    & 36.2                          &  \cellcolor{green!10}$\downarrow$ 0.0\%                 \\
&                                   & DuQuant                          & 70.7                    & 20.7                   & 45.7          & \cellcolor{green!10}$\uparrow$ 0.4\%                      & 33.5                        & 38.8                    & 36.2                          & \cellcolor{green!10}$\downarrow$ 0.0\%                 \\ \cmidrule{2-11} 
& \multirow{3}{*}{W4A4}             & SmoothQuant                      & 0.3                     & 2.0                    & 1.2           & \cellcolor{red!10}$\downarrow$ 97.4\%                         & 0.0                         & 0.0                     & 0.0                           & \cellcolor{red!10}$\downarrow$ 100.0\%               \\
&                                   & QuaRot                           & 62.9                    & 15.2                   & 62.9          & \cellcolor{red!10}$\downarrow$ 14.1\%                               & 23.8                        & 34.6                    & 29.2                          & \cellcolor{red!10}$\downarrow$ 19.3\%                \\
&                                   & DuQuant                          & 64.4                    & 14.8                   & 39.6          & \cellcolor{red!10}$\downarrow$ 13.0\%                         & 25.6                        & 33.6                    & 29.6                          & \cellcolor{red!10}$\downarrow$ 18.1\%                \\ \midrule
\multirow{7}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}LLaDA-8B\\ -Instruct\end{tabular}}} 
& FP Model                          & -                                & 78.5                    & 33.5                   & 56.0          & -                              & 37.8                        & 37.4                    & 37.6                          & -                     \\ \cmidrule{2-11} 
& \multirow{3}{*}{W8A8}             & SmoothQuant                      & 78.2                    & 33.3                   & 55.7          & \cellcolor{green!10}$\downarrow$ 0.4\%                       & 37.2                        & 37.1                    & 38.6                          & \cellcolor{orange!10}$\downarrow$ 1.3\%                \\
&                                   & QuaRot                           & 78.9                    & 33.1                   & 78.9          & \cellcolor{green!10}$\uparrow$ 0.1\%                      & 35.4                        & 36.6                    & 36.0                          & \cellcolor{orange!10}$\downarrow$ 4.3\%                 \\
&                                   & DuQuant                          & 78.1                    & 33.3                   & 55.7          & \cellcolor{green!10}$\downarrow$ 0.5\%                       & 37.2                        & 37.4                    & 37.3                          & \cellcolor{green!10}$\downarrow$ 0.8\%                 \\ \cmidrule{2-11} 
& \multirow{3}{*}{W4A4}             & SmoothQuant                      & 2.7                     & 2.4                    & 2.6           & \cellcolor{red!10}$\downarrow$ 95.4\%                        & 0.0                         & 0.6                     & 0.3                           & \cellcolor{red!10}$\downarrow$ 99.2\%                \\
&                                   & QuaRot                           & 75.1                    & 29.9                   & 75.1          & \cellcolor{red!10}$\downarrow$ 6.2\%                        & 32.3                        & 32.8                    & 32.6                          & \cellcolor{red!10}$\downarrow$ 13.4\%                 \\
&                                   & DuQuant                          & 77.3                    & 30.7                   & 54.0          & \cellcolor{orange!10}$\downarrow$ 3.5\%                      & 34.8                        & 29.2                    & 32.0                       & \cellcolor{red!10}$\downarrow$ 14.9\%                \\ 
\bottomrule
\end{tabular}
}
\end{center}
% \vspace{-1.8em}
\label{tab:wa-math-code}
\end{table*}








\subsection{Optimal Quantization Methods (RQ2)}


\paragraph{GPTQ Outperforms AWQ on Most Tasks}


As shown in Table~\ref{tab:weight-only-general}, GPTQ outperforms AWQ on average accuracy under both 3-bit and 4-bit quantization for LLaDA-8B and LLaDA-8B-instruct. This demonstrates the reliability and competitiveness of GPTQ, particularly on QA tasks.
This trend also holds for math reasoning tasks, except for the 3-bit quantization setting on LLaDA-8B, where both GPTQ and AWQ suffer critical performance degradation (>10\%).
We hypothesize that the suboptimal performance of AWQ may stem from the fact that activation outliers in the LLaDA model series are less prominent than in traditional LLMs. 
Since AWQ identifies the top 1\% of salient weights using activation-driven statistics, its effectiveness can be reduced when the outlier structure is weak in LLaDA models, thereby diminishing its advantage.
For code generation tasks, the situation becomes more complex. Both GPTQ and AWQ fail to maintain acceptable performance on the HumanEval and MBPP benchmarks under low-bit quantization. A more detailed analysis of these results is provided in Section~\ref{subsec:task}.
Notably, AWQ performs relatively better than GPTQ in the 3-bit configuration for code tasks, suggesting some resilience under extreme compression.
Considering all evaluations across task types and bit-widths, we recommend GPTQ as the safer and more generally effective choice for weight-only quantization of diffusion-based language models.





\paragraph{Rotation-Based Methods Achieve Leading Performance Under Weight-Activation Quantization.}

For both LLaDA-8B and LLaDA-8B-instruct, rotation-based methods—QuaRot and DuQuant—consistently outperform SmoothQuant across all evaluation tasks and quantization settings.
The advantage becomes especially pronounced under 4-bit weight-activation quantization, where SmoothQuant suffers a near-complete performance collapse on code and math tasks. In contrast, rotation-based approaches retain a non-trivial portion of model capability, highlighting their robustness in low-precision settings.
These results suggest that rotation transformations are more effective in mitigating activation outliers in dLLMs, which aligns with findings from prior studies in the LLM community~\citep{lin2024duquant,ashkboos2024quarot}.
When comparing QuaRot and DuQuant in detail, our experiments show that DuQuant consistently outperforms QuaRot across most scenarios.
For instance, on commonsense QA tasks, DuQuant achieves lower performance drops than QuaRot for both LLaDA-8B (5.1\% vs. 6.6\%) and LLaDA-8B-instruct (2.5\% vs. 3.9\%).
This observation remains consistent across math and code generation tasks.
Consequently, we recommend DuQuant as the most effective method for weight-activation quantization in diffusion-based language models.


\begin{table*}[!t]
\caption{
Evaluation of weight-only quantized Dream-7B on general tasks.
}
\vspace{-10pt}
\begin{center}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{c|c|c|cccccc}
\toprule
\textbf{Model}                     & \textbf{Setting}            & \textbf{Method} & \textbf{WinoGrande} & \textbf{PIQA} & \textbf{ARC-C} & \textbf{ARC-E} & \textbf{Avg} & \textbf{Drop} \\ \midrule
\multirow{5}{*}{\textbf{Dream-7B}} & FP Model                    & -               & 68.4                & 74.4          & 59.0           & 83.1           & 71.2         & -             \\ \cmidrule{2-9} 
& \multirow{2}{*}{W4A16 g128} & GPTQ            & 68.2                & 73.9          & 58.1           & 82.1           & 70.6         & \cellcolor{green!10}$\downarrow$ 0.8\%         \\
&                             & AWQ             & 65.2                & 69.6          & 55.8           & 82.0           & 68.2         & \cellcolor{red!10}$\downarrow$ 4.3\%         \\ \cmidrule{2-9} 
& \multirow{2}{*}{W3A16 g128} & GPTQ            & 63.3                & 69.6          & 49.9           & 73.4           & 64.1         & \cellcolor{red!10}$\downarrow$ 10.1\%        \\
&                             & AWQ             & 62.8                & 67.7          & 50.6           & 74.5           & 63.9         & \cellcolor{red!10}$\downarrow$ 10.3\%        \\ \bottomrule
\end{tabular}
}
\end{center}
% \vspace{-1.8em}
\label{tab:dream}
\end{table*}


\subsection{Influence of Task Categories on Quantization (RQ3)}
\label{subsec:task}


\paragraph{Quantization is More Challenging for Math and Code Tasks.}

Compared to general-purpose benchmarks—primarily QA tasks as shown in Table~\ref{tab:weight-only-general} and Table~\ref{tab:wa-general}—quantized models experience significantly larger performance drops on math and code tasks, illustrated in Table~\ref{tab:weight-only-math-code}
and Table~\ref{tab:wa-math-code}.

For \textbf{math reasoning} tasks, both AWQ and GPTQ exhibit substantial degradation under 3-bit quantization (see Table~\ref{tab:weight-only-math-code}), despite maintaining competitive performance on general QA benchmarks. A similar trend is observed for rotation-based methods under W4A4 configurations.
This degradation may be attributed to the multi-step reasoning nature of math problems, which amplifies the cumulative effect of quantization errors. In such tasks, precise intermediate representations are critical; even small perturbations introduced by low-bit quantization can propagate and compound, ultimately leading to incorrect final answers.

In \textbf{code generation} tasks, the challenges are even more pronounced. Under 4-bit quantization, GPTQ and AWQ show performance drops exceeding 5\%, while QuaRot and DuQuant degrade by over 10\% under W4A4 for both LLaDA-8B and LLaDA-8B-instruct models. 
We also observe that the standard deviation on the HumanEval benchmark is relatively high, approximately 3\%, indicating that more robust and stable benchmarks may be needed to accurately assess code generation capabilities under quantization.
Code generation tasks often require the model to maintain long-range context and generate syntactically correct, semantically meaningful sequences. These demands are highly sensitive to the precision of both weights and activations. Quantization-induced distortion in attention patterns or token representations can disrupt code syntax or logic, causing severe performance degradation.

These observations highlight that math and code tasks impose stricter precision requirements than simpler retrieval-based or classification-style QA tasks. Maintaining accurate intermediate states, multi-hop logic, and long-context dependency are especially vulnerable under aggressive quantization.
Consequently, task-specific quantization strategies or adaptive precision control mechanisms may be necessary to improve the robustness of dLLMs on math and code benchmarks. This represents a critical direction for future research in efficient diffusion-based LLM deployment.


\subsection{Impact of Model Types (RQ4)}

\paragraph{Instruct-Tuned Models are More Robust than Base Models.}

We observe an interesting phenomenon: LLaDA-8B-instruct consistently exhibits smaller performance degradation than its base counterpart (LLaDA-8B) under nearly all quantization settings.
For instance, under general tasks, both DuQuant and QuaRot result in only minor accuracy drops for the instruct model, whereas the drop exceeds 5\% for the base model.
This trend remains consistent across more challenging math and code tasks.
For example, 3-bit quantized GPTQ and AWQ lead to performance degradation of approximately 5\% for the instruct variant, while the base model suffers drops as high as 10\%.





\textbf{Our Observations Hold Consistently across Different dLLMs.}
To assess the generality of our findings, we further evaluate various quantization methods on a different diffusion-based language model: Dream-7B.
As shown in Table~\ref{tab:dream}, both GPTQ and AWQ perform competitively under 4-bit quantization, while performance drops become more pronounced in the 3-bit setting. 
This observation reinforces our recommendation that 4-bit quantization offers a near-lossless trade-off between efficiency and performance.
Moreover, GPTQ consistently outperforms AWQ across nearly all benchmarks, suggesting that GPTQ is a more reliable choice across different types of dLLMs.
Notably, the 3-bit quantized models exhibit risk-level degradation even on general tasks, indicating that aggressive quantization may be more challenging for the Dream model series compared to LLaDA.
Due to resource constraints, we did not evaluate weight-activation quantization for Dream-7B. We leave this for future work as part of our ongoing exploration.







==> tables/channel-layer.tex <==
 % The results demonstrate the superiority of channel-wise quantization for both INT4 and INT8 weights. The channel-wise approach maintains performance close to the original FP model, whereas the layer-wise approach leads to a noticeable degradation.

% \begin{table*}[!t]
% \caption{\textbf{Comparison of layer-wise and channel-wise quantization on OpenVLA.}
% }
% \label{tab:layer_channel_comparison}
% \centering
% \setlength{\tabcolsep}{4pt}
% \resizebox{0.99\linewidth}{!}{%
% \begin{tabular}{c|cc|cccc|c}
%     \toprule
%         \multirow{2}{*}[-0.5ex]{Weight Type} & \multicolumn{2}{c|}{Quantization Method} & \multirow{2}{*}[-0.5ex]{LIBERO-Spatial} & \multirow{2}{*}[-0.5ex]{LIBERO-Object} & \multirow{2}{*}[-0.5ex]{LIBERO-Goal} & \multirow{2}{*}[-0.5ex]{LIBERO-Long} & \multirow{2}{*}[-0.5ex]{Average} \\[0.3ex]
%     \cline{2-3} 
%         & \rule{0pt}{2.4ex} \hspace{1ex} Layer \hspace{1ex} & \hspace{0.5ex} Channel \hspace{0.5ex} & & & & & \\
%     \midrule
%         FP Model & -- & -- & 84.7\% & 88.4\% & 79.2\% & 53.7\% & 76.5\% \\
%     \midrule
%         \multirow{2}{*}{INT4} & \checkmark & & 84.2\% & 86.8\% & 77.0\% & 51.2\% & 74.8\% \\
%         & & \checkmark & 86.0\% & 88.6\% & 78.4\% & 52.8\% & 76.5\% \\
%     \midrule
%         \multirow{2}{*}{INT8} & \checkmark & & 84.0\% & 87.2\% & 77.8\% & 50.6\% & 74.9\% \\
%         & & \checkmark & 86.2\% & 88.4\% & 79.4\% & 53.1\% & 76.8\% \\
%     \bottomrule
%   \end{tabular}
% }
% \end{table*}


\begin{table*}[!t]
\caption{\textbf{Comparison of layer-wise and channel-wise quantization.}
}
\label{tab:layer_channel_comparison}
\centering
\setlength{\tabcolsep}{4pt}
\resizebox{0.6\linewidth}{!}{%
\begin{tabular}{c|cc|cccc|c}
    \toprule
        \multirow{2}{*}[-0.5ex]{Weight Type} & \multicolumn{2}{c|}{Method} & \multirow{2}{*}[-0.5ex]{Spatial} & \multirow{2}{*}[-0.5ex]{Object} & \multirow{2}{*}[-0.5ex]{Goal} & \multirow{2}{*}[-0.5ex]{Long} & \multirow{2}{*}[-0.5ex]{Avg.} \\[0.3ex]
    \cline{2-3} 
        & \rule{0pt}{2.4ex} \hspace{0.5ex} Layer \hspace{0.5ex} & \hspace{0.5ex} Channel \hspace{0.5ex} & & & & & \\
    \midrule
        FP Model & -- & -- & 84.7\% & 88.4\% & 79.2\% & 53.7\% & 76.5\% \\
    \midrule
        \multirow{2}{*}{INT4} & \checkmark & & 84.2\% & 86.8\% & 77.0\% & 51.2\% & 74.8\% \\
        & & \checkmark & 86.0\% & 88.6\% & 78.4\% & 52.8\% & 76.5\% \\
    \midrule
        \multirow{2}{*}{INT8} & \checkmark & & 84.0\% & 87.2\% & 77.8\% & 50.6\% & 74.9\% \\
        & & \checkmark & 86.2\% & 88.4\% & 79.4\% & 53.1\% & 76.8\% \\
    \bottomrule
  \end{tabular}
}
\end{table*}
